VCG Under False-name Attacks: a Bayesian Analysis

VCG is a classical combinatorial auction that maximizes social welfare. However, while the standard single-item Vickrey auction is false-name-proof, a major failure of multi-item VCG is its vulnerability to false-name attacks. This occurs already in the natural bare minimum model in which there are two identical items and bidders are single-minded. Previous solutions to this challenge focused on developing alternative mechanisms that compromise social welfare. We re-visit the VCG auction vulnerability and consider the bidder behavior in Bayesian settings. In service of that we introduce a novel notion, termed the granularity threshold, that characterizes VCG Bayesian resilience to false-name attacks as a function of the bidder type distribution. Using this notion we show a large class of cases in which VCG indeed obtains Bayesian resilience for the two-item single-minded setting.

==> WIP.tex <==
We want to show that omitting a 2-type always helps the truthful bid relative to the attack, and that adding a 1-type as well always helps the truthful bid relative to the attack. 

\begin{example}
Consider true type $(2,0.2)$ and attack $(1,0.3),(1,0.3)$ faced with adversary $(1,0.3),(2,0.4)$. Then both utilities are $0$. Consider we omit $(2,0.4)$. Then truthful bid utility is $0$, attack utility is $-0.2$. This shows that omitting a 2-type bid doesn't always hurt the attacker. 
\end{example}


==> meetings.tex <==
additional issues:

1) Prove the dominance for theta=1 among split attacks. 

2) Example 6.3 works with 0.2 in the support (w.p. epsilon)? make sure. 

3) Rerun 5.2 simulations (for 2-types, with parameter x in the polynomial). Also look for counter examples for q* monotonicity. 

4) For 2-types and any distribution, the split attack $q^*$ is higher than any other attack. (4a -> 5 given appendix F) WRONG, counter example in notes, I should write it. (Also can serve as a counter-example for A.5)
The counter example analysis is in the Mathematica file: 2-type\_attack\_better\_than\_split. The example is where per-item values are drawn w.p. half from either 0.3 or 1. The true type is $(2,0.4)$ and the attack is $x=y=0.7$. The split attack in this setting has $q^* = 1/6 (8 - \sqrt{46}) \approx 0.202945$. But the attack specified has a much higher $q^* = \frac{1}{2}$. 

5) Add to the affiliation of Ron that he is also at the U. of Bath, UK.

6) Widen the latex margins and check that no mathematical formula significantly exceeds the margins (mainly equations 3 and 5).

7) Prepare a draft for a detailed response to the comments

====

Introduction and abstract (maybe also the intro or conclusions):

1) *DONE* fix the incorrect impression of R2 “a negative results saying that for three or more bidders, truthful BNE only exists in very limited cases” to “a negative result saying that for three or more bidders, truthful BNE does not exist in *all* cases”

2) *DONE* We need to admit more explicitly that the model is limited and state why is it still interesting. Two main reasons are: a) the most general case is not correct so one has to develop some natural restrictions and we believe that our analysis is an important first step. b) our analysis is general enough to allow us to develop

3) *DONE* some high level conclusions:

3a) initially we thought that the case of two bidders will be the hardest since there should be some monotonicity and if for some n there is truthful BNE then for all larger n there will be truthful BNE. Our results show this is not the case. Why?? Develop a high-level explanation.
(check section 4, the graphs in section 5 show that this is the rule, not the exception

3b) After the examples discuss some observations regarding attacks that are beneficial, for example, it can be beneficial to attack even if a player wants just one item, split attack, maybe more?

4) *DONE* the family of distributions in sec 5 includes all $f(x)=a*x^{a-1}$ for any integer $a \geq 1 (CDF F(x)=x^a)$.

5) *DONE* Other BNEs: explain why truthfulness is the probable BNE, if it is indeed a BNE.

6) *DONE* refer to the new discussion section.

*DONE* AE: one recommendation is that it would be helpful to use the numerical simulations to surface some economic insights about the problem and/or its solution.  Does the exercise tell us anything, at a high level, about false-name proofness in auctions or the cost of mitigating the impact of false-name bids?

Regarding R1 (mention also in the cover letter):
1) R1’s report states “providing negative results would be compelling”. We do provide negative results so we need to emphasize that in the letter and the paper.
2) R1 did not understand the rationale behind the definition of the granularity threshold (again we need to explain in the paper and mention in the letter).
3) We need to admit more explicitly that the model is limited and state why is it still interesting.


==> meetings_old.tex <==
Agenda for next meeting:
- Go over the example for 3.
- Go over 2b analysis.

additional issues:

-2) Prove the dominance for theta=1 among split attacks. 

-1) Example 6.1 works with 0.2 in the support (w.p. epsilon)? make sure. 

0) Rerun 5.2 simulations (for 2-types, with parameter x in the polynomial). 

1) where should we place example 6.1?

Extensions and open question: (add to the discussion)

monotonicity

1) the monotonicity of $q^*_{F(alpha,beta)}$, even just for beta=1. We do not know.

2) monotonicity of q (if for some q truthfulness is BNE then this holds for any q'>q). We do not know, but the natural sufficient condition for this is wrong (i.e. sometimes when the adversary has more 2-types it is less beneficial to attack).

2a) Monotonicity of q for the split attack (this would generalize Lemma E.1, that shows it specifically for the uniform distribution). I WROTE A PROOF SKETCH, which is now Lemma E.1. 

2b) Show non-monotonicity of q based on Example 6.1 for n=3. We do not know.

It is possible to find F and attack(x,y) such that the function is positive at q=0. For example, take F that chooses 0.5 w.p. 1, a true type (2,1), and an attack x=y=0.1. Then the true utility is 1, and the attack utility is 0. But in this case, facing a mix of 1-type and 2-type adversaries, the true utility is again 1, and the attack utility is again 0, and so there is still monotonicity. So it's important to look for the more sophisticated conditions. For these conditions, I do think it's a difficult question.

additional structural attempts

3) maybe: for all $n,\theta,x,y,F$, $q^*_{n,g=2,\theta,x,y,F} \geq q^*_{n,g=1,\theta,x,y,F}$. We have a counter example - WRITE IT DOWN (it's not example 6.1). 

a small change to example 6.1 works (instead of comparing the attack x=1,y=0.2 for a (1,1) with the split attack for a (2,1), compare it with the same attack (x=1,y=0.2) for a (2,1)). 


4) For any distribution, the split attack $q^*$ is higher than any other attack. We have a counter example (same as above).

4a) For 2-types and any distribution, the split attack $q^*$ is higher than any other attack. (4a -> 5 given appendix F) WRONG, counter example in notes, I should write it. (Also can serve as a counter-example for A.5)

5) For the uniform distribution, the split attack $q^*$ is higher than any other attack. This will imply that q*(UNI) = 1/2. We do not know (we know how to prove it for $g=1$ and in our empirical analysis it was correct for all $n$'s we tested).

Introduction and abstract (maybe also the intro or conclusions):

1) fix the incorrect impression of R2 “a negative results saying that for three or more bidders, truthful BNE only exists in very limited cases” to “a negative result saying that for three or more bidders, truthful BNE does not exist in *all* cases”

2) We need to admit more explicitly that the model is limited and state why is it still interesting. Two main reasons are: a) the most general case is not correct so one has to develop some restrictions and we believe that our analysis is an important first step. b) our analysis is general enough to allow us to develop some high level conclusions:

2a) initially we thought that the case of two bidders will be the hardest since there should be some monotonicity and if for some n there is truthful BNE then for all larger n there will be truthful BNE. Our results show this is not the case. Why?? Develop a high-level explanation.

2b) After the examples discuss some observations regarding attacks that are beneficial, for example, it can be beneficial to attack even if a player wants just one item, split attack, maybe more?

3) the family of distributions in sec 6 includes all $f(x)=a*x^{a-1}$ for any integer $a \geq 1 (CDF F(x)=x^a)$.

4) Other BNEs: explain why truthfulness is the probable BNE, if it is indeed a BNE.

AE: one recommendation is that it would be helpful to use the numerical simulations to surface some economic insights about the problem and/or its solution.  Does the exercise tell us anything, at a high level, about false-name proofness in auctions or the cost of mitigating the impact of false-name bids?

Regarding R1 (mention also in the cover letter):
1) R1’s report states “providing negative results would be compelling”. We do provide negative results so we need to emphasize that in the letter and the paper.
2) R1 did not understand the rationale behind the definition of the granularity threshold (again we need to explain in the paper and mention in the letter).
3) We need to admit more explicitly that the model is limited and state why is it still interesting.

